WEIZZ: Automatic Grey-box Fuzzing for Structured Binary Formats

Fuzzing technologies have evolved at a fast pace in recent years, revealing bugs in programs with ever increasing depth and speed. Applications working with complex formats are however more difficult to take on, as inputs need to meet certain format-specific characteristics to get through the initial parsing stage and reach deeper behaviors of the program. Unlike prior proposals based on manually written format specifications, in this paper we present a technique to automatically generate and mutate inputs for unknown chunk-based binary formats. We propose a technique to identify dependencies between input bytes and comparison instructions, and later use them to assign tags that characterize the processing logic of the program. Tags become the building block for structure-aware mutations involving chunks and fields of the input. We show that our techniques performs comparably to structure-aware fuzzing proposals that require human assistance. Our prototype implementation WEIZZ revealed 16 unknown bugs in widely used programs.

==> background.tex <==
% !TEX root = main.tex

\section{Background}

\subsection{American Fuzzy Lop}

American Fuzzy Lop (AFL) is a widely used grey-box coverage guided fuzzer.

It employs genetic algorithms and program instrumentation to store
generated inputs that trigger new program states.

It relies on instrumentation for both source code or binaries to log the coverage
in terms of edges and times that such edges are hit during the traced execution.

That information is logged in shared memory between the fuzzer and the target program.

Programs states are approximated with the notion of {\em hitcounts} of and edge.
To avoid path explosion the times that an edge is hit is mapped in several buckets
representing the hitcounts:

1, 2, 3, 4-7, 8-15, 16-31, 32-127, 128+

If an input reaches one of this hitcounts for the first time it is considered
interesting for AFL.

For the input generation, AFL makes use of several fuzzing strategies.
The early stages are deterministic, for example, the input is bit flipped,
known interesting integers like 0 or -1 are placed sequentially in the inputs
or small integers are sequentially added or subtracted.

After the deterministic steps, AFL applies random stacked mutations in the so-called
{\em havoc} stage. The mutations are random bitflips, insertion, deletion, copying of a portion
of the input and arithmetics.

The number of executions of the havoc stage on a testcase is determinated by a
performance score evaluated using the execution latency and the testcase size.

As of the last resource, if the previous stages failed to discover new interesting inputs,
the testcase is merged with another random testcase from the queue of the fuzzer
and then the same mutations of havoc are applied in the so-called {\em splicing} stage.

To match magic bytes and approximate the grammar of an input format, the user
can specify a set of keywords in a user-supplied dictionary.
Those strings are sequentially inserted in the deterministic stages and
randomly inserted and appended in the random stages.

\subsection{Fuzzing Roadblocks}

% riassunto su Vuzzer / Redqueen che bypassano usando magic bytes e su QSYM / Driller / Eclipser che usano hybrid fuzzing

\subsection{Smart Greybox Fuzzing}

Smart Greybox Fuzzing (SGF) is a recent technique that introduces a new set of
mutational operators based on the virtual structure of the file rather than
on the bit level representation. These operations aim to generate
an almost valid new input and explore new input domains.

AFLSmart is is the proposed implementation of SGF based on the widely
used binary file format fuzzer American Fuzzy Lop.

In AFLSmart, the virtual structure is a generic and lightweight data structure
that is adapted to describe different file formats.
Each input is represented using a tree in which each node is a chunk (internal
nodes) or an attribute (leaves).
Each chunk has a start and end index in the file and an associated type.
An attribute is the basic unit and is not structurally relevant by its own
but only when related to other attributes.

AFLSMart uses the File Cracker component of Peach to build the virtual structure
of an input using the probabilistic deferred parsing strategy because of the
parsing process can steal a lot of time to fuzzing.
The probability that the parser is invoked increase with the time since the
the last path is discovered.

The added mutations that make use of the virtual structure are:

\begin{itemize}
  \item Smart Deletion: delete a random chunk
  \item Smart Addition: choose a random chunk from an arbitrary taken second input and add after a chunk in the current input that has the same parent.
  \item Smart Splicing: choose a random chunk, take a chunk with the same type from an arbitrary second input and substitute the first chunk with the second.
\end{itemize}

These mutations generate files that likely more valid than files generated with
bit-level mutations but strict validity is not a guarantee.

AFLSmart introduces also a power schedule based on the validity of a testcase.
The degree of validity is the percentage of the file that is successfully parsed.
The energy assigned to a testcase is doubled if its validity is at least 50\%.


==> evaluation-orig.tex <==
% !TEX root = main.tex

\section{Evaluation}
\label{se:evaluation}

%We evaluated our implementation of \ourname to answer the following research questions:
%We sought evidence for the following research questions:
We now present the results of a three-pronged evaluation of our prototype to address the following research questions:
\begin{itemize}
  \item {\bf RQ 1.} How does \ourname compare to state-of-the-art fuzzers %when considering
on targets that process chunk-based formats?\smallskip %Is \ourname effective even in absence of format specifications?
  \item {\bf RQ 2.} Can \ourname identify new bugs?%real-world applications?
  \smallskip
  \item {\bf RQ 3.} How do tags relate to the actual input formats? And what is the role of structural mutations and roadblock bypassing in the observed improvements?
  %Are the improvements from \ourname due to structural mutations, roadblock bypass techniques, or both of them?    
\end{itemize}

To answer these questions, we divide our evaluation into three parts.\note{Droppare se poco spazio}
%
First, we compare the code coverage achieved by \ourname and several state-of-the-art fuzzers on the targets reported in Table~\ref{tab:targets}: these applications process chunk-based formats and have been used in the past to evaluate prominent fuzzers (e.g.,\cite{aflsmart-tse}, \cite{ECLIPSER-ICSE19}, and~\cite{vuzzer}). Our experiments show that \ourname can achieve high code coverage on these targets, even when compared to \aflsmart that requires a format specification %in order to be able 
to perform chunk-based mutations.\note{valutare se essere piu' aggressivi}

Second, we show how \ourname is not only able to achieve high code coverage on real-world applications, but it can also find new bugs. \ourname discovered 10 novel bugs inside well-tested software, such as Apple CUPS and the GNU coreutils utility {\tt objdump}.

Finally, we dig into our experiment results, analyzing a few case studies to demonstrate that tags --- although placed through heuristics --- can actually be strongly related to the actual format of an input and that structural mutations are actually crucial for the effectiveness of \ourname. 

\subsubsection*{Experimental setup} The experiments were conducted on a server equipped with two Intel\textsuperscript{\textregistered} Xeon\textsuperscript{\textregistered} E5-4610 v2 @ 2.30GHz with 8 cores each and 256 GB RAM, running Debian Linux 9.2. To compare different fuzzers, we measured the basic block coverage achieved for each fuzzer by running the target application over the entire set of inputs generated by the fuzzer, computing the cumulative coverage across different executions. We repeated each experiment five times, plotting in the charts the median value and reporting in the tables ranges based on a 60\% confidence interval~\cite{redqueen}. In the second stage of \ourname, we set Pr$_{field} =\ $Pr$_{chunk} = 1/15$: this is consistent with the probability used by \aflsmart at applying smart mutations. % instead of other mutations from \afl when fuzzing a target. 
Finally, to avoid \ourname from spending excessive time at bit flipping large inputs, we restricted the first stage to inputs with less than 3000 bytes.%, excluding with the exception of the ffmpeg runs in which we set the limit to 8000 bytes because our initial seed is an AVI of 6000 bytes circa.

We plan to fully release our experimental setup, alongside the source code of \ourname, possibly helping other researchers to rerun our experiments in the future.

\begin{table}[t]
  \caption{Target applications considered in the evaluation: top 6 in Section~\ref{ss:comparison-aflsmart} and bottom 8 in Section~\ref{ss:comparison-other-fuzzers}.\label{tab:targets}}
  \begin{adjustbox}{width=0.7\columnwidth,center}
  \small
  %\centering
  \begin{tabular}{ |l|l|l| }
    \hline
    {\sc Program} & {\sc Release} & {\sc Input Format} \\
    \hline\hline
    wavpack & {\tt 5.1.0} & WAV \\
    decompress (openjp2) & {\tt 2.3.1-git} & JP2 \\
    ffmpeg & {\tt 4.2.1} & AVI \\
    \hline
    libpng  & {\tt 1.6.37} & PNG \\
    readelf (GNU binutils) &  {\tt 2.3.0} &  ELF  \\
    djpeg (libjpeg-turbo) & {\tt git:5db6a68} & JPEG \\
    \hline
    objdump (GNU binutils) & {\tt 2.32.51} & ELF \\
    mpg321  & {\tt 0.3.2} & MP3 \\
    oggdec (vorbis-tools) & {\tt 1.4.0} & OGG  \\
    tcpdump & {\tt 4.9.2} & PCAP \\ % 4.9.2 (libpcap 1.8.1)
    gif2rgb (GIFLIB) & {\tt 5.2.1} &  GIF \\
    \hline
    
    \hline
  \end{tabular}
  \end{adjustbox}
\end{table}

\subsection{Targets processing chunk-based formats}
\label{ss:eval-coverage}

To answer RQ 1, we evaluate the effectiveness in terms of code coverage provided by \ourname on the targets reported in Table~\ref{tab:targets}. Since \ourname mainly targets applications that process chunk-based formats, we start by discussing a detailed comparison against \aflsmart: this is a state-of-the-art smart greybox fuzzer which specifically targets this class of programs. Indeed, \aflsmart implements chunk-based mutations that, given a specification of the format processed by an application, can fuzz the input based on its {\em virtual} structure (see Section~\ref{se:related}). 

We then extend our comparison by considering other state-of-the-art fuzzers, that although not equipped with smart mutations, can be still be effective in practice on this kind of targets, as shown by past works, e.g.,\cite{aflsmart-tse} and~\cite{ECLIPSER-ICSE19}.

\subsubsection{\bfseries{\scshape{Weizz}} versus \bfseries{\scshape{AFLSmart}}} 
\label{ss:comparison-aflsmart}

For this comparison, we consider the top 6 applications from Table~\ref{tab:targets}. These targets process 6 distinct input formats (right column in Table~\ref{tab:targets}) and have been considered in past evaluations involving \aflsmart.\note{Motivare perche' abbiamo scelto 6 su 12?} To enable smart mutations in this fuzzer, we provided to \aflsmart the peach pits developed and publicly released by its authors for these formats.

% \note{quali seed? i seed sono presi o dal set di AFL o da https://github.com/mathiasbynens/small}

We measured the code coverage achieved by: (a) \aflsmart, using its latest release at the time of experiments (commit {\tt 604c40c}) and configuring it with stack mutations but without deterministic stages, as suggested by its authors in the project documentation, (b) \ourname, using its standard configuration, %hence enabling all the features described in Section~\ref{se:methodology} and Section~\ref{se:implementation}, 
and (c) {\ourname}$^{\dagger}$, a variant of \ourname, where operand fuzzing ({\sc FuzzOperands}), checksum patching ({\sc PatchAllChecksums}), and input fixing ({\sc FixChecksums}) have been disabled. We included {\ourname}$^{\dagger}$ in order to evaluate the effect on code coverage due to tag-based mutations, discarding any additional benefit provided by the roadblocks bypass techniques integrated into \ourname, which are not available in \aflsmart. Nevertheless, to help both \aflsmart and {\ourname}$^{\dagger}$ deal with magic numbers, we provided to them dictionaries containing %common
tokens from the input formats under fuzzing, consistently with past evaluations of \aflsmart. As initial seeds, we considered testcases from \afl, while only for wavpack and ffmpeg we used samples %taken 
from the {\sc small} project~\cite{small-files-project} which provides {\em the smallest possible syntactically valid files} for several formats.

\iffalse
\begin{itemize}
  \item \aflsmart: latest release at the time of writing (commit {\tt 604c40c}), configured to run stack mutations but disabling the deterministic stages (as suggested in the project {\tt README});
  \item \ourname: standard configuration, enabling all the features described in Section~\ref{se:methodology} and Section~\ref{se:implementation};
  %\ast
  \item {\ourname}$^{\dagger}$: same configuration as \ourname but disabling operand fuzzing ({\sc FuzzOperands}), checksum patching ({\sc PatchAllChecksums}), and input fixing ({\sc FixChecksums}): this makes it possible to evaluate the impact of tag-based mutations, without benefiting from the roadblocks bypass techniques integrated into \ourname (which are not available in \aflsmart).
\end{itemize}
\fi

\begin{figure}[t]
  %\vspace{0.5cm}
  \centering
  \adjustbox{max width=0.82\columnwidth}{
  \input{evaluation3}
  }
  \vspace{-1mm}
  \begin{table}[H]
    \footnotesize
    \centering
    \begin{tabular}{ l l l }
     \fcolorbox{black}[HTML]{4363D8}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \weizz & \fcolorbox{black}[HTML]{E6194B}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \aflsmart & \fcolorbox{black}[HTML]{3CB44B}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad {\weizz}$^{\dagger}$ \\ 
    \end{tabular}
  \end{table}
  \vspace{-3mm}
  \caption{Basic blocks coverage (median) over time (5 hours) for the top 6 subjects listed in Table~\ref{tab:targets}.\label{fig:comparison-aflsmart}}% for \ourname, \aflsmart, and {\ourname}$^{\dagger}$.
\end{figure}

% (even sometimes significantly as shown by the experiment on wavpack)
Figure~\ref{fig:comparison-aflsmart} plots the median basic block coverage when running the targets for 5 hours under \ourname, \aflsmart, and {\ourname}$^{\dagger}$, while Table~\ref{tab:comparison-aflsmart-ci} (Appendix~\ref{appendix-eval}) reports the 60\% confidence intervals for the coverage at the end of our experiments.
%To evaluate the statistical significance of these results, we also report in Table~\ref{tab:comparison-aflsmart-ci} (Appenfix~\ref{appendix-eval}) the 60\% confidence intervals for the basic block coverage reached at the end of our experiments. 
Overall, when comparing \ourname to \aflsmart, the former provides significantly higher code coverage on 3 out of 6 subjects (readelf, libpng, and ffmpeg), it slightly improves coverage on wavpack, it is comparable on decompress, and it performs slightly worse on djpeg. To understand these results, we should first consider the coverage achieved by {\ourname}$^{\dagger}$ and then evaluate the benefits that comes due to additional features available \ourname.

% weizzX vs aflsmart: tag-based mutations seems to work really well. Why? weizz muta strutturalmente in base a come il porgramma handles input bytes, andando a lavorare solo su byte manipolati. questo gli permette di fare mutazione che vanno oltre quanto indicato dalla specificato, possibilmente facendo emergere bug dell'implementazione. Gia' aflSMART riconosce che rilassare la specifica porta a trovare comportamente interessanti, grimoire usa questo come un selling point.
% weizzX vs weizz: sfruttare input-to-state puo' aiutare ad identificare costanti non presenti nei dizionari o addirittura non presenti nella specifica (incompleta e legata ad un singolo formato). Weizz grazie input-to-state riesce a fuzzare bene anche programmi multi formato quando in combinazione con le tag mutations. Inoltre, le tecniche di roadblocks bypass sono utili ad esempio in libpng.

The improvement in coverage between {\ourname}$^{\dagger}$ and \aflsmart comes from the different approaches in devising structural mutations. While the latter structurally mutates the input based on the format specification, \ourname structurally mutates the input based on {\em how} the program handles the input bytes. Hence, it is able to reveal program behaviors that are due to the actual implementation of the input parser and could not be necessarily predicted by reasoning over the specification. This has two main implications. First, \ourname applies mutations focusing on the part the input that is actually relevant for the program, reasoning over tags that are strongly connected to the execution of comparison instructions from the program. Second, the imprecision in understanding the input structure can actually benefit \ourname. Indeed, even \aflsmart has recognized that relaxed specifications can actually help a fuzzer when looking for bugs due to imprecise implementations~\cite{aflsmart-tse}. A similar consideration has been recently also pointed out by \grimoire, which similarly to \ourname does not fuzz inputs based on a format specification. 

%These results suggest that \ourname is not only able to mutate the input as effectively as \aflsmart even without requiring an input format specification, but it benefits significantly from the roadblocks bypass techniques that it integrates. Indeed, when considering {\ourname}$^{\dagger}$, we can see that, although dictionaries containing magic numbers can help during fuzzing\footnote{We remark that \aflsmart can infer magic bytes both from the format specification and from the dictionaries. However, dictionaries are used only in the havoc stage, are not exhaustive (we used the same dictionaries as in the evaluation of \aflsmart) and do not provide insights on where to place the magic numbers within the input.}, they are less effective than operand-based mutations such as the ones performed by {\sc FuzzOperands}. A crucial consideration is that while \aflsmart mutates the structure of the input based on the format specification, it does not perform the mutations based on how the implementation of the input parser under test actually {\em behaves} when processing the input, i.e., it blindly assumes that mutating the structure of an input can increase the code coverage. Conversely, \ourname first evaluates the behavior of the program in terms of comparison instruction execution and then it possibly structurally mutates the part of the input that is relevant for the program computation (i.e., it infers the structure based on the tags placed due to comparison instructions). Hence, {\sc FuzzOperands} does not only target magic numbers from the format but also reveals other checks which the program may integrate for its own logic, that could not be exposed by the format specification.

%Another crucial difference that may help at making \ourname more effective than \aflsmart is that while the latter can spend a significant amount of time for reconstructing the input model (as reported by its authors in~\cite{aflsmart-tse}), the former is designed to fuzz while learning the structure of an input: for instance, {\sc GetDeps} identifies input dependencies while fuzzing at the same time the program, possibly contributing in the code coverage.

Additional benefits emerge when including the roadblock bypass techniques into the picture. \ourname improves in terms on coverage over {\ourname}$^{\dagger}$ for two main reasons: input-to-state fuzzing and checksum bypass techniques. The former helps {\ourname} {\em learn} constants, such as magic numbers, possibly missing in the dictionaries or the format specification, significantly supporting it when fuzzing programs handling multiple input formats, such as ffmpeg. On the other hand, the latter is crucial to generate valid inputs for programs that verify the integrity of the input data. A relevant example is provided by libpng which verifies chunks using CRC-32 checksums.


In Table~\ref{tab:comparison-best-alternative}\note{Drop questa o l'altra tabella se poco spazio}, we compare \ourname with the best alternative in terms of code coverage for each of the 6 targets. We can see that in the worst case \ourname is at most 4\% worse than the best alternative and for one target is able to achieve up to 32\% more coverage. When taking into account possible crashes detected during our evaluation, while all three fuzzers were able to generate the same set of crashes for wavpack, on the other hand, only \ourname was able to crash ffmpeg. This is not surprising when considering that ffmpeg can process multiple input formats and \ourname is designed to generate inputs that could even diverge significantly from the initial seed (e.g., mutating a AVI file into a MPEG-4 file). In Section~\ref{se:real-world-bugs}, we will present a few case studies that further support this claim. In the case of ffmpeg, we verified that the crash is due to a division by zero located into a code section handling multiple formats. We reported the bug to the developers of ffmpeg, which promptly fixed it in the master branch.

\subsubsection{\bfseries{\scshape{Weizz}} versus other greybox fuzzers}
\label{ss:comparison-other-fuzzers}

\begin{table}[t]
  \centering
  \caption{\ourname vs the best alternative for each target from Figure~\ref{fig:comparison-aflsmart}: a percentage of basic block (BB) coverage higher (lower) than 100\% means that \ourname is better (worse) than the best alternative.\label{tab:comparison-best-alternative}}
  \begin{adjustbox}{width=0.75\columnwidth,center}
  \small
  \begin{tabular}{ |l||c|c|c| }
    \hline
  \thead{\sc Programs} & \thead{\sc Best\\\sc Alternative} & \thead{\sc\% of BBs\\\sc w.r.t. the Best} & \thead{\sc Crashes\\\sc found by}\\
    \hline
    wavpack & \aflsmart & 106\% & all\\
    readelf & {\ourname}$^{\dagger}$ & 110\% & none \\
    decompress & \aflsmart & 100\% & none \\
    djpeg & \aflsmart & 96\% & none \\
    libpng & {\ourname}$^{\dagger}$ & 132\% & none \\
    ffmpeg & {\ourname}$^{\dagger}$ & 114\% & \weizz \\
    \hline
  \end{tabular}
  \end{adjustbox}
\end{table}

\begin{figure}[t!]
  %\vspace{0.5cm}
  \centering 
 \adjustbox{max width=0.8\columnwidth}{
  \input{evaluation1}
  }
  \vspace{-1mm}
  \begin{table}[H]
    \footnotesize
    \centering
    \begin{tabular}{ c c c c }
     \fcolorbox{black}[HTML]{4363d8}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \weizz & \fcolorbox{black}[HTML]{FF9966}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \eclipser & \fcolorbox{black}[HTML]{3cb44b}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \aflpp & \fcolorbox{black}[HTML]{e6194b}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \afl
    \end{tabular}
  \end{table}
  \vspace{-3mm}
  \caption{Basic blocks coverage (median) over time (24 hours) for the bottom 8 subjects listed in Table~\ref{tab:targets}.\label{fig:comparison-other-fuzzers}}
\end{figure}

After comparing with \aflsmart, we extend the evaluation of \ourname by considering other state-of-the-art fuzzers that have shown to be effective on targets processing chunk-based formats. For this set of experiments, we executed the bottom 8 programs from Table~\ref{tab:targets}: these are popular open source applications, heavily fuzzed from the community (e.g., through OSS-Fuzz~\cite{google-oss-fuzz}, a Google project aimed at continuous fuzzing of open source software), and have been used in past evaluations of state-of-the-art fuzzers (e.g.,~\cite{aflsmart-tse,vuzzer,Li:2017:SPB:3106237.3106295,redqueen}).

Beside \ourname, we tested the following fuzzers: (a) \afl 2.53b in QEMU mode, (b) \aflpp 2.54c in QEMU mode, enabling the CompareCoverage feature, %in order to support sub-instruction profiling
(c) \eclipser, using its latest release at time of writing (commit {\tt 8a00591}) and its default configuration. We did not consider any fuzzer requiring source instrumentation, such as \angora, since \ourname targets binary programs. We could not run \steelix since it is no publicly available, but we instead considered \aflpp with the CompareCoverage feature enabled, as one of the best binary fuzzers integrating sub-instruction profiling. Finally, we could not include \redqueen in our experimental comparison for two main reasons: it is not yet publicly available at the time of writing and it builds on top of the Intel PT tracing extensions, making unfair to compare it with a fuzzer, such as \ourname, based on the standard QEMU, that inherently would incur a significant larger overhead compared to tracing framework based on Intel PT, regardless of the methodology devised by the fuzzer. We refer the reader to Section~\ref{se:discussion} for a conceptual comparison with \redqueen and to Section~\ref{se:tag-impact} for an experiment where we configure \ourname to conceptually match the features in \redqueen.

% A subset of these targets (3 out of 8) have been considered also in Section~\ref{ss:comparison-aflsmart}, providing a mean for indirectly comparing \aflsmart with other fuzzers considered in this set of experiments.

As emerged in the comparison with \aflsmart, %checks due to magic numbers and internal logic from a target may a have huge impact on the code coverage when evaluating a fuzzer. Nonetheless, 
structural mutations are likely to play a crucial role when considering applications processing chunk-based formats. Hence, since  \afl, \aflpp and \eclipser lack the support for smart mutations, we opted to run the 8 targets for 24 hours, a larger budget w.r.t. the experiments involving \aflsmart, possibly allowing these fuzzers to compensate the lack of this feature over time and recover in terms of code coverage. Consistently with previous evaluations~\cite{ECLIPSER-ICSE19}, we used as initial seed for 6 out of 8 targets a string containing 72 times the ASCII character "0". For libpng and tcpdump, we had to use two {\em meaningful} initial inputs\footnote{For libpng, we used the {\tt not\_kitty.png} testcase from \afl, while for tcpdump, we captured a few seconds of traffic during a Capture-The-Flag competition.} since no fuzzer, excluding \ourname, was able to achieve significant code coverage when using artificial seeds. Finally, to help \afl bypassing magic numbers, we provided to this fuzzer dictionaries containing format-specific tokens.

Figure~\ref{fig:comparison-other-fuzzers} plots the median basic block coverage over time when testing the 8 targets with different fuzzers, while Table~\ref{tab:comparison-other-fuzzers-ci} (Appendix~\ref{appendix-eval}) reports the 60\% confidence intervals for the basic block coverage at the end of the 24-hours experiments. On 5 out 8 targets (i.e., libpng, oggdec, tcpdump, objdump and readelf), \ourname achieves significantly higher code coverage than other fuzzers. The formats processed by libpng, oggdec, and tcpdump contain input checksums, which can be bypassed only by \ourname (although \eclipser appears to catch up over time when looking at oggdec): this reason and the ability to perform structural mutations explain the gap in terms of coverage between \ourname and other fuzzers. When considering objdump and readelf, the result likely derives from the ability of \ourname at identifying input-to-state dependencies (even resulting from string comparators) and fuzz them through {\sc FuzzOperands}\note{Daniele: check this}: this is consistent with the experiments reported by \redqueen~\cite{redqueen} on these two targets.
%indirectly confirmed by the experiments involving these two targets in the evaluation of \redqueen~\cite{redqueen}, which suggest a similar conclusion. 

%from the structural mutations integrated into \ourname. We further elaborate on the experiment involving readelf in Section~\ref{se:tag-impact} in order to support this claim. 

On mpg321 and gif2rg, fuzzers based on \afl perform very similarly, showing a significant gap with respect to \eclipser, and confirming that standard mutations from \afl can be quite effective even on chunk-based formats. Finally, \ourname is the best on djpeg, although other fuzzers are not too far in terms of coverage. 

Table~\ref{tab:comparison-fuzzers-best-alternative} compares \ourname with the best alternative fuzzer in terms of code coverage for each target. Interestingly, on 3 out of 8 targets, \afl is the best alternative to \ourname, performing significantly better than other fuzzers especially when considering libpng. \eclipser outperforms \aflpp and \afl on oggdec and tcpdump, but falls short on mpg321 and gif2rgb. When taking into account crashes (shown in the right column of Table~\ref{tab:comparison-fuzzers-best-alternative}), \ourname and \aflpp both generated known crashing inputs for mpg321, while \ourname is the only fuzzer that revealed a crash for objdump (see Section~\ref{se:real-world-bugs} for more details).

%This hypothesis behind this result is indirectly confirmed when considering the previous set of experiment, where \aflsmart was only slightly worse in terms of coverage with respect to \ourname.

\begin{table}[t]
  \centering
  \caption{\ourname vs the best alternative for each target from Figure~\ref{fig:comparison-other-fuzzers}: a percentage of basic block (BB) coverage higher (lower) than 100\% means that \ourname is better (worse) than the best alternative.\label{tab:comparison-fuzzers-best-alternative}}
  \begin{adjustbox}{width=0.8\columnwidth,center}
  \small
  \begin{tabular}{ |l||c|c|c| }
    \hline
    \thead{\sc Programs} & \thead{\sc Best\\\sc Alternative} & \thead{\sc \% of BBs\\\sc w.r.t. Best} & \thead{\sc Crashes\\\sc found by}\\
    \hline
    djpeg & \afl & 105\% & none \\
    libpng & \afl & 180\% & none \\
    objdump & \aflpp & 120\% & \weizz \\
    mpg321 & \aflpp & 100\% & \weizz, \aflpp\\
    oggdec & \eclipser & 108\% & none\\
    readelf & \aflpp & 175\% & none\\
    tcpdump & \eclipser & 117\% & none\\
    gif2rgb & \afl & 100\% & none\\
    \hline
  \end{tabular}
  \end{adjustbox}
\end{table}

\subsection{Zero-day bugs}
\label{se:real-world-bugs}

\begin{table}[t]
  \caption{Bugs found and reported in real-world software.\label{tab:bugs}}
  \centering
  \begin{adjustbox}{width=0.85\columnwidth,center}
  \small
  \begin{tabular}{ |l|l|l| }
    \hline
    Program & Bug ID & Type \\
    \hline
    objdump (GNU binutils) & Bugzilla \#24938 & CWE-476\\
    CUPS (Apple) & rdar://problem/50000749 & CWE-761\\
    CUPS (Apple) & GitHub \#5598 & CWE-476\\
    libmirage (CDEmu) & CVE-2019-15540 & CWE-122\\
    libmirage (CDEmu) & CVE-2019-15757 & CWE-476\\
    dmg2img & Launchpad \#1835461 & CWE-476\\
    dmg2img & Launchpad \#1835463 & CWE-125\\
    dmg2img & Launchpad \#1835465 & CWE-476\\
    jbig2enc & GitHub \#65 & CWE-476\\
    mpg321 & Launchpad \#1842445 & CWE-122\\
    ffmpeg & Ticket \#8335 & CWE-369\\
    \hline
  \end{tabular}
  \end{adjustbox}
\end{table}

A crucial feature of \ourname is that it does not require an input format specification when fuzzing a program, allowing users to easily analyze quite different applications without requiring any significant manual effort. %Indeed, although if \ourname provides structural mutations as \aflsmart, it is able to automatically infer the structure of an input and mutates it revealing new interesting 
To demonstrate the effectiveness of \ourname, we ran it on several different targets, even involving applications that process inputs that do not strictly fall within the chunk-based class of formats. Overall, \ourname was able to reveal 11 zero-day bugs in 7 popular and well-tested applications: 6 bugs involve NULL Pointer Dereferences (CWE-476), one bug allows an attacker to free a non-heap buffer (CWE-761), 2 bugs can lead to buffer overflows (CWE-122), one bug generates an out-of-bounds read (CWE-125), and one bug generate a division by zero (CWE-369). The full list of bugs is provided in Table~\ref{tab:bugs} and in the remainder of this section we present the details on three bugs that provide interesting insights on the effectiveness and versatility of \ourname. We remark that most of the crashes identified during the experiments presented in Section~\ref{ss:eval-coverage} involve known bugs and thus are not covered in this section.

\subsubsection*{Apple CUPS}
% Attraverso una richiesta HTTP, attaccante puo' far cambiare un puntatore in una struct. Tale puntatore normalemente fa riferimento a un blocco allocato dinamicamente, mentre con l'attacco puo' essere fatto puntare verso un blocco non in heap, permettendo exploit di tipo house of spirit, visto che CUPS effettua una realloc.
% interessante perchè mostra come weizz e' in grado di essere efficace anche su programmi non strettamente chunk based come HTTP

The Common UNIX Printing System (CUPS) is an open source project, currently owned and developed by Apple, that provides a print spooler and job scheduler on the majority of UNIX-like operating systems. Users can interact with the CUPS server through requests in the Hypertext Markup Language (HTML) in order to configure printers, submit jobs, and alter the queue status. Although HTML cannot be dubbed as a chunk-based input format, we tested whether \ourname could still be able to perform valuable mutations when generating HTTP requests against CUPS. Interestingly, \ourname was able to automatically craft a request that led the CUPS server to reallocate a user-controlled buffer not contained in the heap, paving the road to a {\em House of Spirit} attack~\cite{house-of-spirit}. The key to find the bug was to first insert into a request the {\tt Accept-Language} field through {\sc FuzzOperands} and then duplicate it via chunk mutations. The bug has been confirmed by Apple and fixed in the release {\tt 2.3b8}. As an additional evidence on the effectiveness of \ourname at crafting HTTP requests for this target, we reported also to Apple a NULL-pointer dereference that has been later fixed in the release {\tt 2.3.0}.

\subsubsection*{libMirage} The libMirage library provides uniform access to data stored in several disk image formats, such as IMG, ISO, and NRG. \ourname was able to identify a critical bug in its code: an attacker can generate a heap-based buffer overflow, which in turn has the potential to corrupt the allocator metadata and even possibly lead to root access for the attacker since the vulnerable code is used by the CDEmu daemon that runs with root privileges on most Linux systems. An interesting insight behind this bug is that \ourname was fed with an ISO image as the initial seed, while it ended spotting a bug within the NRG image parser, demonstrating how \ourname can deviate even considerably from one input format to another one based on how the program handles the input bytes.

\subsubsection*{objdump}
% NULL pointer dereference, interessante perche' parte da ELF e arriva a toccare codice relativo a PE

The GNU binary utilities, commonly known as {\em binutils}, are one of the most tested suite of programs from the security community, e.g., via the OSS-Fuzz project from Google. Nonetheless, \ourname was able to detect a NULL pointer dereference inside objdump, a powerful tool for displaying information about one or more binary objects. Similarly to libMirage, it was surprising to verify that the bug is contained in a piece of code that handles the Portable Executable (PE) format, while the initial seed provided to \ourname was a  Extensible Linking Format (ELF) binary.

%\subsubsection*{ffmpeg}
% division by zero, interessante perchè' in modo simile a  objdump identifica un bug in un pezzo di codice che opera su piu' formati

\subsection{Understanding the impact of tags}
\label{se:tag-impact}

%The previous sections have shown that \ourname can be effective at covering new code when considering targets processing chunk-based file formats as well as finding bugs in well-tested software. 
A compelling question is {\em why} \ourname is effective at fuzzing applications that process chunk-based file formats. Unfortunately, understanding the root causes is far from being a trivial task since targets may implement very different approaches when processing input bytes, often even working on quite diverse formats. Nonetheless, we attempt to partially answer this question by considering two case studies: first we evaluate whether tags generated by \ourname on one seed for libpng can actually support field and chunk identification during the structure-aware stage of \ourname, then we show that both tag-based mutations and roadblocks bypass techniques are essential for \ourname on ffmpeg, demonstrating that none of these features alone is enough to reach the same coverage achieved by \ourname.

% show that the kind of structural mutations carried out by \ourname are indeed crucial when fuzzing programs considered in our evaluation, focusing on ffmpeg, which is one of the targets where \ourname provides significantly higher code coverage than \aflsmart.

\subsubsection*{Tag accuracy} Figure~\ref{fig:weizz-png} shows the raw bytes from the initial seed ({\tt not\_kitty.png} testcase) used when fuzzing libpng. The testcase starts with a 8-bytes magic number (i.e., {\tt PNG\_SIGNATURE}, in orange) and then contains 5 chunks. Each chunk is characterized by four fields: the length (4 bytes, in green), the type (4 bytes, red), the chunk data (which could contain different kinds of data, such as {\tt PNG\_CHUNK\_IDR} in yellow, {\tt IDAT\_DATA} in grey, {\tt PNG\_CHUNK\_TEXT LABEL} in purple followed by {\tt PNG\_CHUNK\_TEXT DATA} in lilac, and {\tt PNG\_CHUNK\_PLTE} in teal blue), and the CRC-32 checksum (4 bytes, in blue). The last chunk has no data since it used merely as a marker for the end of the PNG.

To evaluate whether \ourname can actually identify the different fields in a PNG file, we analyzed the tags placed by the {\sc SurgicalFuzzing} stage on the {\tt not\_kitty.png} testcase, running repeatedly the heuristic for finding field boundaries: after detecting the end of the first field (starting from the first byte of the testcase), we restarted the heuristic to find the spatially next field, repeating this process until the of the file was reached. %\footnote{Since most fields in {\tt not\_kitty.png} match the first pattern presented in Section~\ref{se:tag-mutations}, \ourname could find most of the fields by running several times the field heuristic with completely random start positions.}. 
Fields identified from \ourname are delimited in square brackets in Figure~\ref{fig:weizz-png}, while bytes tagged as part of a checksum field are shown as underlined. \ourname was able to identify most PNG fields with correct boundaries with a few exceptions. The last three fields in the file are not recognized at all since they are part of the last chunk, which is never accessed by libpng. The length fields (green color) is split by \ourname into different fields: libpng tests this field using different comparison instructions at different execution times, making hard for \ourname to detect the field boundaries. Some data fields, such as {\tt PNG\_CHUNK\_IDR}, are merged with the spatially next CRC-32 checksum: although inaccurate from the point-of-view of the format specification, the merge make sense since the comparison instruction verifying the CRC-32 has dependencies both over the CRC-32 field and the data field. Nonetheless, \ourname correctly marks the bytes in the CRC-32 as checksum fields, allowing it to possibly fix them through {\sc FixChecksums}. Finally, {\tt IDAT DATA} can be regarded as a binary blob that is fragmented by \ourname into distinct fields (with gaps among them due to untagged bytes) since its bytes are processed by several different routines that do not necessarily perform compare operations on the entire set of bytes from this blob. 

Assessing whether \ourname can identify precisely chunk boundaries is considerably more tricky. The heuristic for identifying chunks can be quite sensitive to the starting position from which it starts analyzing tags. For instance, when starting from the PNG magic number, it is able to correctly capture the entire testcase as an outer chunk. Similarly, when starting from one of the bytes in a {\tt LENGTH} field, it may been able to capture all the other fields from that chunk\footnote{Depending on the starting byte, it could miss some of the first bytes.}. However, when for instance starting from a byte of the {\tt TYPE} field, it could fail to consider within the boundaries other fields from that chunk. Nonetheless, even when chunk boundaries are not detected precisely with respect to the format specification, \ourname can still perform valuable structural mutations for two main reasons. First, structural mutations, such as adding or splicing, insert bytes from another testcase that are hopefully {\em consistent} with the original ones, e.g., splicing looks for a chunk of the same {\em type}, possibly resulting in a valid input even when wrongly detecting the chunk boundaries. Second, as previously pointed out by \grimoire in the context of grammar-based fuzzing, this kind of inaccuracy can actually be beneficial in terms of coverage and bugs identification since it may expose program behaviors that are not well-tested from the developers since they are due to inputs that do not perfectly conform to the specification. When considering the libpng program, \ourname is indeed able achieve higher code than other fuzzers (see Section~\ref{ss:eval-coverage}), even compared to \aflsmart which performs smart mutations guided by a format specification.


\begin{figure}[t]
  \centering
  \vspace{-1.5mm}
  \includegraphics[width=70mm]{png_format_weizz}
  \caption{Fields identified by \ourname on the {\tt not\_kitty.png} testcase when fuzzing libpng.\label{fig:weizz-png}}
\end{figure}

\begin{figure}[t]
  %\vspace{0.5cm}
  \centering
  
  \adjustbox{max width=0.75\columnwidth}{
  \input{evaluation2}
  }
  \vspace{-1mm}
  \begin{table}[H]
    \footnotesize
    \centering
    \begin{tabular}{ c c c c }
     \fcolorbox{black}[HTML]{4363d8}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \weizz & \fcolorbox{black}[HTML]{3cb44b}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad {\ourname}$^{\dagger}$ & \fcolorbox{black}[HTML]{FF9966}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad {{\weizz}$^\ddagger$} & \fcolorbox{black}[HTML]{e6194b}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \aflsmart
    \end{tabular}
  \end{table}
  \vspace{-3mm}
  \caption{Fuzzing ffmpeg for 5 hours: \ourname vs {\weizz}$^\dagger$ (no roadblocks bypass techniques) vs {\weizz}$^\ddagger$ (no tag-based mutations) vs \aflsmart.\label{fig:impact-tag-mutations}}
\end{figure}

\subsubsection*{Structural mutations vs roadblock bypass} When considering experiments from Section~\ref{ss:eval-coverage}, one natural question may emerge: {\em Is the improvement in terms of code coverage due to the structural mutations or due to the roadblocks bypass techniques?} To shed light on this question, we consider the ffmpeg target and compare three configurations of our fuzzer: (a) \ourname, the full-fledged version, (b) {\weizz}$^\dagger$, a variant where roadblock bypass techniques have been disabled, and (c) {\weizz}$^\ddagger$, a variant where tag-based mutations have been disabled\footnote{This variant is the one that better resemble \redqueen from a methodological point-of-view.}. The code coverage and input queue size during 5 hour experiments from these fuzzers\footnote{We also show the coverage from \aflsmart for reference. We do not report its queue size since it handles inputs quite differently w.r.t. \ourname.} are depicted in Figure~\ref{fig:impact-tag-mutations}. When picking only one feature between tag-based mutations and roadblock bypass techniques, we can see that on ffmpeg the former is more effective (+17\%) than the latter in terms of code coverage. This is surprising since ffmpeg supports multiple formats and input-to-state dependencies are crucial to learn new magic numbers and unlock several program paths. Nonetheless, structural mutations from \ourname are indeed essential on ffmpeg. When combining both of these features into \ourname, we get the best result, reaching a +34\% in coverage with respect to {\weizz}$^\ddagger$. Interestingly, the queue size of {\weizz}$^\dagger$ is larger than the one from \ourname: this means that although \ourname explore more branches from the program, {\weizz}$^\dagger$ covers some of the branches more exhaustively, i.e., it is able to cover more hit count buckets for some branches.

%To further support our claim that the structural mutations carried out by \ourname, although not always conformant with the format specification, are indeed crucial for achieving high code coverage for our fuzzer, we discuss an additional experiment involving ffmpeg. In Section~\ref{ss:comparison-aflsmart}, we have shown that \ourname achieves considerably more code coverage than \aflsmart, raising one natural question: {\em is the improvement due to the structural mutations or due to the roadblocks bypass techniques?} To shed light on this question, we compare \ourname against {\weizz}$^\ddagger$, a variant where tag-based mutations from the second stage have been disabled\footnote{This variant is the one that better resemble \redqueen from a methodological point-of-view.}. Figure~\ref{fig:impact-tag-mutations} depicts the basic block coverage and the queue size during a 5-hours experiment. \ourname not only achieves higher code coverage (134\%) than {\weizz}$^\ddagger$ but it is also characterized by a larger queue over time, demonstrating that it generates more {\em interesting} inputs (which result from improving branch hit counts). %Hence, the structural mutations are indeed crucial for \ourname when considering ffmpeg.



\iffalse
\subsubsection*{RQ 1} Is our technique more effective and efficient than
other state-of-the-art binary-only fuzzers on chunks-based file formats?

\subsub{section*{RQ 2} Is our technique comparable to Smart Grey-Box Fuzzing when the
specification of the input format is available?

\subsubsection*{RQ 3} Are the tags-based mutations improvements for our technique?

\subsubsection*{RQ 4} Are the generated tags meaningful concerning the input structure? \\

To evaluate the performance of a fuzzer we use the Basic Blocks coverage metric like
previous works in literature.
This is an estimation of the effectiveness of a fuzzer because if a fuzzer cannot
explore a portion of code cannot find bugs in that code.
We do not list the number of crashes because is a not well-defined metric, instead
we list if a fuzzer generated at least one true positive crash.
Assertion errors are not listed.

% The reported Edge coverage is not context-sensitive so that to have a fair evaluation
% with all other fuzzers.

We used a patched version of user-mode QEMU with an instrumentation similar to the one
used by the various tested fuzzers to log the coverage.
This tool runs the tested binaries with all the testcases in the queue of the evaluated fuzzers as input.

This version of \qemu is compatible with the checksums patching methodology of \weizz
and does not need to have all the inputs in the queue fixed.
We made sure to run this tracer only after the fuzzing process in order to not
log the coverage generated by the false-positive checksums.

We runned each experiment for 5 times and then we computed the median value of the logged data
and the confidence intervals of 60\%. The median is reported in graphs to show the progress
of the fuzzers, the intervals are reported only for the final coverage.

% comment: use http://www.learningaboutelectronics.com/Articles/Confidence-interval-calculator.php

For the entire evaluation, we set the Pr$_{field}$ and Pr$_{chunk}$ probabilities both to
1/15 that is a bit more than the probability assigned by \aflsmart to its
structural mutations when stacking them with the \afl mutations (1/17).





All the experiments were run on a machine with 32 Intel(R) Xeon(R) CPU E5-4610 v2 2.30GHz
and 252 GB of RAM.

\subsection{State of the art binary-only fuzzers}

To answer RQ1, we evaluated the performance in terms of basic blocks coverage
in comparison to three state-of-the-art binary-only fuzzers on well-fuzzed programs that parse structured inputs.

The fuzzers are:

\begin{itemize}
  \item \afl 2.53b with the \qemu instrumentation, because the \weizz implementation is based on this fuzzer;
  \item \aflpp 2.54c with the \qemu instrumentation and the CompareCoverage option enabled, as one of the most advanced binary-only fuzzers publicly available;
  \item \eclipser, as the binary-only fuzzers with the most advanced branch-solving technique available at the time of writing.
\end{itemize}

We do not evaluate RedQueen because, at the time of writing, this fuzzer is not publicly available.

For a fair comparison, we provided a dictionary with the relevant magic bytes to \afl because all the other fuzzers can bypass magic bytes with their respective techniques.

This explains the performance of \afl over \eclipser in some targets.

We ran \eclipser alternating Grey-Box concolic testing with random fuzzing using the default
configuration. This configuration may be not optimal for all targets but we did not
manually tune any fuzzer for specific targets apart from the dictionary for \afl.

We run \aflpp with the CompareCoverage level 2 that instruments all comparisons not only comparisons
with immediates, like \weizz does. CompareCoverage is a binary-only feature for QEMU
similar in spirit to laf-intel that allow \aflpp to solve roadblocks.

We also limited the {\em getdeps} stage to process testcases with a size not greater than 3000 bytes
to avoid to spend a high percentage of the 24 hours in bit flipping large inputs.

% This, however, is not so necessary because \weizz performs the input trimming before passing it to {\em getdeps}.

We run each fuzzer for 24 hours for each binary.
All the fuzzers started from a common seed input, the ASCII character \verb|0| for 72 times, except for libpng
and tcpdump because all other fuzzers except \weizz were not able to produce significant results.
For libpng we used the \verb|not_kitty.png| image from the \afl testcases set and a small PCAP for tcpdump.
They will be both published with the source code of \weizz to enable future evaluations.

Note that the libpng binary is a test harness based on the libpng default example.

The results of the in terms of Basic Blocks discovered each second are shown in Figure 1.

In Table 1 we compare the final Basic Blocks coverage and Edge coverage of each tested fuzzer.
We also list the fuzzers that found at least one bug during the 24 hours evaluation.
All of those programs are well-fuzzed and continuously tested with frameworks like OSS-FUZZ
and during the evaluation time, we were able to crash only two programs of the eight, mpg321 and objdump.

In all the tests \weizz results the best fuzzer in terms of Basic Blocks and Edge coverage also on targets that do not have checksums checks like djpeg.
\fi


\iffalse % PPH
\begin{table}[H]
  \footnotesize
  \centering
  \begin{tabular}{ l l }
   \fcolorbox{black}[HTML]{4363d8}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \weizz & \fcolorbox{black}[HTML]{3cb44b}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \aflpp QEMU CompareCoverage \\
   \fcolorbox{black}[HTML]{ff9966}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \eclipser & \fcolorbox{black}[HTML]{e6194b}{\rule{0pt}{2pt}\rule{2pt}{0pt}}\quad \afl QEMU with dictionary \\  
  \end{tabular}
\end{table}
\fi

\iffalse
In this section, the fuzzers are feed with a minimal seed. Each seed is the smallest
valid file that we were able to produce for each tested format.

To evaluate the improvement given by the tags based mutations
we tested two versions of \weizz on the ffmpeg target for 5 hours as a use case.
The first version is simply \weizz and the second,
\weizz$^1$, is \weizz without tags mutations.

% For this test the logged edges coverage is context-sensitive.

% insert this before the \end{picture} in evaluation2.tex
% \put(2490,1144){\fcolorbox{black}[HTML]{e6194b}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad \weizz}
% \put(2490,884){\fcolorbox{black}[HTML]{3cb44b}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad \weizz$^1$}



\iffalse
\begin{table}[h]
  \centering
  \caption{Basic Blocks Coverage Intervals of confidence}
  \begin{tabular}{ |c|c| }
    \hline
    \weizz & {\weizz}$^\ddagger$ \\
    \hline
    {\bf 15946-17885} & 12071-12983 \\
    \hline
  \end{tabular}
\end{table}
\fi

The \weizz basic blocks coverage in 5 hours of ffmpeg fuzzing
is the 134\% of the \weizz$^1$ basic blocks coverage.
The Queue size related to the Tags mutations is 174\% of the other.
Despite that, this is not a metric that can, in general, evaluate fuzzers efficiency,
when it is used to compare two similar fuzzers it highlights the ability to discover hitcounts.

\fi

\iffalse
While in terms of basic block and edges coverage the two fuzzers seems to start to converge in the last
part of the graph, the \weizz queue continuously grow suggesting that it is discovering new hitcounts.

The results show that the tags mutations are an improvement in terms of coverage
and a hitcounts and that the choice to use context-sensitive edge coverage due to the presence of the
higher-level mutations is reasonable.
\fi
\iffalse
For further evaluation of the tags methodology, we compared a version of \weizz
with only tags mutations enabled against the Smart Grey-Box fuzzing implementation \aflsmart
and the version of \weizz with all features enabled.
We disabled surgical mutations and checksums patching to have a fair evaluation
on programs that have checksum checks and magic bytes not listed in the dictionary
provided to \aflsmart by its authors.
Always for fairness, we provided the same dictionary to this version of our fuzzer, \weizz$^2$, that so
now performs only the getdeps stage, the tags construction, and the random mutations.
% We expect that a fuzzer that rely on a manually specified structure like \aflsmart
% outperforms our approach based on tags.

\aflsmart runs with the deterministic stages disabled and stack mutations enabled, as suggested in its README.
The dictionaries used are taken from the \aflsmart repository \footnote{https://github.com/aflsmart/aflsmart}.

We run the experiments on 6 programs that are a subset of the programs used in the
\aflsmart experiments, one for each file format tested in the \aflsmart paper.
% \weizz can learn tags about multiple formats but \aflsmart uses a structure
% specification of only one file format at a time.

The chosen file formats are WAV, ELF, JP2, JPEG, PNG, AVI and, respectively, the programs are
wavpack, readelf jasper, djpeg, libpng, FFmpeg.


\begin{table}[h]
  \centering
  \caption{Basic Blocks and Edge coverage Intervals of confidence}
  \begin{tabular}{ |l||c|c|c|c| }
    \hline
    Programs & \multicolumn{2}{c|}{BBs Coverage Intervals} & \multicolumn{2}{c|}{Edge Coverage Intervals} \\
    \hline
     & \aflsmart & \weizz$^2$ & \aflsmart & \weizz$^2$ \\
    \hline
    wavpack & 1499-1642 & 1700-1759 & 2158-2395 & 2464-2557 \\
    readelf & 6087-6188 & 6586-6731 & 10494-10700 & 11458-11718 \\
    libpng & 1001-1036 & 1189-1232 & 1333-1391 & 1589-1660 \\
    \hline
  \end{tabular}
\end{table}




As you can see in Figure 3, surprisingly \weizz in at least one of its versions
outperforms \aflsmart on four of the six tested programs.
% The difference in libpng is very high and are probably because
% we apply tags mutations also in the splicing stage.

There a many factors that can explain these results. We did not disabled the context-sensitive coverage and our structural mutations are performed also in the splicing stage.
\aflsmart, instead, apply the structural mutations only in the havoc stage.

Regards the FFmpeg case, instead, \weizz can learn and mutate the tags describing
different file formats and \aflsmart is limited only to one of them, AVI.

On the other hand, \weizz$^2$ has a dictionary limited to the AVI magic bytes and without
the surgical mutations cannot reach the code that parses other formats.

The results of this third part of our experiment suggest that the answer to
RQ3 is that \weizz is comparable to \aflsmart on programs that parse
binary file formats.

Another interesting fact that can be observed from this results is that sometimes \weizz$^2$
outperforms \weizz. This is due to the dictionary that not only give some free magic bytes to the
fuzzer but prevent also te fuzzer to spend a significant amount of time in surgical mutations.

In the fuzzer implementation, each feature can be surgically disabled with command line
options to let the user choose the best configuration when there is a knowledge
about the fuzzed program file format.

\subsection{Real World Bugs}

While evaluating the ability of \weizz to discover new paths in the fuzzed programs,
we tested it on well-fuzzed targets to find new bugs.


All the programs parse binary file formats except Apple CUPS,
that is controlled via HTTP requests.
The bug is an invalid reallocation of an heap pointer that is not the starting address of a chunk in the heap. The memory associated with the pointer can be controlled by an attacker to craft a fake chunk and performs an
House fo Spirit attack on realloc.

Our instrumentation extracted all the tokens used to composed an HTTP request.
HTTP, like XML, can be represented with chunks and \weizz (like \aflsmart) can
effectively fuzz it.
However, the set of bit-level mutation was useless and the bugs were discovered
thanks to the fact that to strings discovered using the heavy instrumentation is
then inserted in the extra dictionary.

Another interesting bug is the one found on objdump. It is a Null Pointer Dereference
related to the metadata in the header of the PE format.
This is interesting because the fuzzer was feed with an ELF file and it generated
PE files.

The crashes reported in the previous sections but not here are known bugs.
The wavpack bugs are know bugs and are the same trigghered by \aflsmart in its paper.
\fi

\iffalse
\subsection{File Format VS Tags}

As a case study, we show the relation between a tagged input produced by the first iteration of \weizz
on the libpng target and the PNG file format.

In Figure M the first image is the \verb|not_kitty.png| default testcase of AFL with the
relevant fields of the PNG file formats highlighted. Similar fields (eg. chunk names)
have the same color. The second image is the same
testcase with the fields based on tags of the same type highlighted with the same color \footnote{The one-byte tolerance, as explained in Implementation, is applied}.
White bytes are untagged. The colors between the two images are unrelated.

The checksum fields, in the first picture, are marked with the
color \fcolorbox{black}[HTML]{7da7d8}{\rule{0pt}{1pt}\rule{1pt}{0pt}}.
In the second image, the checksum fields recognized during the first {\sc WeizzFirstStage}
are underlined.

The two checksums fields that are not recognized are not used in libpng.
The first is the checksum of the \verb|tEXt| chunk, not executed thanks to the check that disables checksums check for "ancillary" chunks in \verb|png_crc_error|.
The second is the checksum of the \verb|IEND| chunk, an empty chunk that delimits the end of the PNG.
This part of the input is untagged because never hit \footnotemark, as we observed debugging the application.
\fi

\iffalse
\begin{figure}[h]
  %\vspace{0.5cm}
  \caption{PNG Format Fields and Tags Fields comparison}
  \centering
  \includegraphics[width=50mm]{tabella_png_out}
\end{figure}
\fi

%\footnotetext{The associated routine is png\_handle\_IEND}

